Zeus: A System Description of the Two-Time Winner of the Collegiate SAE AutoDrive Competition

The SAE AutoDrive Challenge is a three-year collegiate competition to develop a self-driving car by 2020. The second year of the competition was held in June 2019 at MCity, a mock town built for self-driving car testing at the University of Michigan. Teams were required to autonomously navigate a series of intersections while handling pedestrians, traffic lights, and traffic signs. Zeus is aUToronto's winning entry in the AutoDrive Challenge. This article describes the system design and development of Zeus as well as many of the lessons learned along the way. This includes details on the team's organizational structure, sensor suite, software components, and performance at the Year 2 competition. With a team of mostly undergraduates and minimal resources, aUToronto has made progress towards a functioning self-driving vehicle, in just two years. This article may prove valuable to researchers looking to develop their own self-driving platform.

==> sections/calibration.tex <==
\section{Calibration}

\begin{itemize}
    \item In Year 1 of the competition, we placed a significant emphasis on calibration.
    \item It’s a hard problem, very few solutions are turn-key, require a lot of domain knowledge and fine-tuning to get them to work properly.
    \item CAM-VEL calibration packages.
    \item Much easier: design your mechanical mounts such that you already know the relative translations and rotations with reasonably high certainty. This was sufficient for us in Year 2 of the competition. We used the expected calibration using hand-measurements and CAD models.
    \item Also easier: design perception algorithms to be robust to minor errors in the calibration. Major errors in calibration are easy for a human to detect using a simple GUI.
    \item We calibrate the relative transformations between sensors in a piece-wise manner.  There are works out there trying to optimize all transformations simultaneously.
    \item Talk about trying to replace our HDL-64 with 4 x VLP-16s.
    \item Calibrating Velodyne to IMU, IMU to rear-wheel-axle frame.
    
\end{itemize}

==> sections/hardware.tex <==
\section{Hardware Design}

\begin{itemize}
    \item Describe roof rack
    Needed a roof rack that would accommodate future sensor suite configurations, be rigid enough so that sensor positions remain relatively constant
    \item Our system is capable of operating in heavy rain, but strategy to weather-proof our system is not elegant. We wrap connections to sensors in plastic to prevent moisture from damaging them.
    \item Our DNNs are robust to minor debris and rain drops on the camera lenses but need to be wiped down occasionally.
    \item Describe electrical design. (Why EVs are nice to work with in comparison with ICE vehicles.
    \item Auxilliary Power Supply in our Chevrolet Bolt supplies up to 1kW of power. Our electrical design routes power from this source to the server, LIDAR, GPS/IMU, and radar.
    \item Intel server is the primary source of power consumption. We don't have GPUs, but if you have serveral GPUs, you may need more than 1KW to power everythuing.
    \item Synch PCB: we implemented a PCB that will allow us to accurately time stamp sensor measurements via the UTC time published by the GPS/IMU.
\end{itemize}
